All-Action Policy Gradient Methods: A Numerical Integration Approach

While often stated as an instance of the likelihood ratio trick [Rubinstein, 1989], the original policy gradient theorem [Sutton, 1999] involves an integral over the action space. When this integral can be computed, the resulting "all-action" estimator [Sutton, 2001] provides a conditioning effect [Bratley, 1987] reducing the variance significantly compared to the REINFORCE estimator [Williams, 1992]. In this paper, we adopt a numerical integration perspective to broaden the applicability of the all-action estimator to general spaces and to any function class for the policy or critic components, beyond the Gaussian case considered by [Ciosek, 2018]. In addition, we provide a new theoretical result on the effect of using a biased critic which offers more guidance than the previous "compatible features" condition of [Sutton, 1999]. We demonstrate the benefit of our approach in continuous control tasks with nonlinear function approximation. Our results show improved performance and sample efficiency.

==> bibrefs.tex <==



@ARTICLE{Aleksandrov1968,
author={Aleksandrov, V.M. and Sysoyev, V.I. and Shemeneva, V.V.},
title={Stochastic optimization},
journal={Engineering Cybernetics},
year={1968},
volume={5},
number={5},
pages={11-16}
}










@inproceedings{Fellows2018,
  author    = {Matthew Fellows and
               Kamil Ciosek and
               Shimon Whiteson},
  title     = {Fourier Policy Gradients},
  booktitle = {Proceedings of the 35th International Conference on Machine Learning,
               {ICML} 2018, Stockholmsm{\"{a}}ssan, Stockholm, Sweden, July
               10-15, 2018},
  pages     = {1485--1494},
  year      = {2018}
}

@book{evans2000,
  title={Approximating integrals via Monte Carlo and deterministic methods},
  author={Michael Evans and Timothy Swartz},
  volume={20},
  year={2000},
  publisher={OUP Oxford}
}


@article{Fujimoto,
  author    = {Scott Fujimoto and
               Herke van Hoof and
               Dave Meger},
  title     = {Addressing Function Approximation Error in Actor-Critic Methods},
  journal   = {CoRR},
  volume    = {abs/1802.09477},
  year      = {2018},
}
@inproceedings{Adam,
  author    = {Diederik P. Kingma and
               Jimmy Ba},
  title     = {Adam: A Method for Stochastic Optimization},
  booktitle = {3rd International Conference on Learning Representations, ICLR 2015,
               San Diego, CA, USA, May 7-9, 2015, Conference Track Proceedings},
  year      = {2015},
}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
